A 4 tonne demonstrator for large-scale dual-phase liquid argon time projection chambers

A 10 kilo-tonne dual-phase liquid argon TPC is one of the detector options considered for the Deep Underground Neutrino Experiment (DUNE). The detector technology relies on amplification of the ionisation charge in ultra-pure argon vapour and oers several advantages compared to the traditional single-phase liquid argon TPCs. A 4.2 tonne dual-phase liquid argon TPC prototype, the largest of its kind, with an active volume of 3x1x1 $m^3$ has been constructed and operated at CERN. In this paper we describe in detail the experimental setup and detector components as well as report on the operation experience. We also present the first results on the achieved charge amplification, prompt scintillation and electroluminescence detection, and purity of the liquid argon from analyses of a collected sample of cosmic ray muons.

==> anames/AuthorList.tex <==
%\author[label1,label2]{Ben Smith\corref{cor1}\fnref{label3}}%% author list to be updated

\newcommand{\INSTA}{\affiliation{\bf ETH Zurich, Institute for Particle Physics, Zurich, Switzerland}}

\newcommand{\INSTBE}{\affiliation{\bf University of Bern, Albert Einstein Center for Fundamental Physics, Laboratory for High Energy Physics (LHEP), Bern, Switzerland}}

\newcommand{\INSTE}{\affiliation{\bf Universit\'e de Lyon, Universit\'e Claude Bernard Lyon 1, IPN Lyon (IN2P3), Villeurbanne, France}}

\newcommand{\INSTJ}{\affiliation{\bf IRFU, CEA Saclay, Gif-sur-Yvette, France}}

\newcommand{\INSTJY}{\affiliation{\bf Department of Physics, University of Jyv\"askyl\"a, Finland}}

\newcommand{\INSTBU}{\affiliation{\bf Faculty of Physics, University of Bucharest, Bucharest, Romania}}

\newcommand{\INSTNCBJ}{\affiliation{\bf National Centre for Nuclear Research (NCBJ), Warsaw, Poland}}

\newcommand{\INSTCE}{\affiliation{\bf CERN, Geneva, Switzerland}}

\newcommand{\INSTLAPP}{\affiliation{\bf LAPP, Universit\'e de Savoie, CNRS/IN2P3, Annecy-le-Vieux, France}}

\newcommand{\INSTPARIS}{\affiliation{\bf UPMC, Universit\'e Paris Diderot, CNRS/IN2P3, Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Paris, France}}

\newcommand{\INSTAPC}{\affiliation{\bf APC, AstroParticule et Cosmologie, Universit\'e Paris Diderot, CNRS/IN2P3, CEA/Irfu, Observatoire de Paris, Sorbonne Paris Cit\'e, 10, rue Alice Domon et L\'eonie Duquet, 75205 Paris Cedex 13, France}}

\newcommand{\INSTUCL}{\affiliation{\bf Dept. of Physics and Astronomy, University College London, London, United Kingdom}}

\newcommand{\INSTCIEMAT}{\affiliation{\bf Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}}

\newcommand{\INSTBARCEL}{\affiliation{\bf Institut de Fisica d'Altes Energies (IFAE), Bellaterra (Barcelona), Spain}}


\newcommand{\INSTKEK}{\affiliation{\bf High Energy Accelerator Research Organization (KEK), Tsukuba,  Ibaraki, Japan}}

\newcommand{\INSTIWA}{\affiliation{\bf Iwate University, Department of Electrical Engineering and Computer Science, Morioka, Iwate, Japan}}

\newcommand{\INSTKUR}{\affiliation{\bf National Institute of Technology Kure College, Kure, Hiroshima, Japan}}

\newcommand{\INSTIFIN}{\affiliation{\bf Horia Hulubei National Institute of R\&D for
Physics and Nuclear Engineering - IFIN-HH, Magurele, Romania}}

\newcommand{\INSTOMEGA}{\affiliation{\bf OMEGA Ecole Polytechnique/CNRS-IN2P3,
route de Saclay,  Palaiseau, France}}

\newcommand{\INSTPRIN}{\affiliation{\bf Princeton University, Princeton, USA}}

\newcommand{\INSTUTA}{\affiliation{\bf University of Texas Arlington, Arlington, USA}}

\newcommand{\INSTFERMI}{\affiliation{\bf Fermilab, Batavia, IL, USA}}

\newcommand{\INSTKYI}{\affiliation{\bf Kyiv National University, Kyiv, Ukraine}}

% Annecy LAL, Annecy
\author{B.\,Aimard}\INSTLAPP
\author{G.\,Balik}\INSTLAPP
\author{L.\,Brunetti}\INSTLAPP
\author{A.\,Chappuis}\INSTLAPP
\author{I.\,De Bonis}\INSTLAPP
\author{C.\,Drancourt}\INSTLAPP
\author{D.\,Duchesneau}\INSTLAPP
\author{N.\,Geffroy}\INSTLAPP
\author{Y.\,Karyotakis}\INSTLAPP
\author{H.\,Pessard}\INSTLAPP
\author{A.\,Remoto}\INSTLAPP
\author{S.\,Vilalte}\INSTLAPP
\author{L.\,Zambelli}\INSTLAPP

%% Texas Arlington
\author{F.~Andrea}\INSTUTA
\author{Ch.~Animesh}\INSTUTA
\author{B.~Garrett}\INSTUTA
\author{Y.~Jaehoon}\INSTUTA
\author{A.~Jonathan}\INSTUTA
\author{S.~Shahsavarani}\INSTUTA

%% Barcelona
\author{B.\,Bourguille}\INSTBARCEL
\author{S.\,Bordoni}\INSTBARCEL
\author{S.~Di~Luise}\INSTBARCEL
\author{T.\,Lux}\INSTBARCEL
\author{F.\,Sanchez}\INSTBARCEL

%% Fermilab
\author{G.\,Brunetti}\INSTFERMI

%% Bern
\author{M.\,Auger}\INSTBE
\author{A.\,Ereditato}\INSTBE
\author{R.\,Hanni}\INSTBE
\author{I.\,Kreslo}\INSTBE
\author{D.\,Lorca}\INSTBE
\author{P.\,Lutz}\INSTBE
\author{J.\,Sinclair}\INSTBE
\author{M.\,Weber}\INSTBE


%% Bucharest
\author{M.\,Calin}\INSTBU
\author{T.\,Esanu}\INSTBU
\author{A.\,Jipa}\INSTBU
\author{I.\,Lazanu}\INSTBU
\author{L.\,Nita}\INSTBU
\author{O.\,Ristea}\INSTBU
\author{C.\,Ristea}\INSTBU

%% CERN
\author{N.\,Bourgeois}\INSTCE
\author{J.\,Bremer}\INSTCE
\author{M.\,Chalifour}\INSTCE
\author{N.\,Charitonidis}\INSTCE
\author{F.\,Duval}\INSTCE
\author{G.\,Lehmann-Miotto}\INSTCE
\author{G.\,Maire}\INSTCE
\author{D.\,Mladenov}\INSTCE
\author{M.\,Nessi}\INSTCE
\author{F.\,Noto}\INSTCE
\author{F.\,Pietropaolo}\INSTCE
\author{F.\,Resnati}\INSTCE
\author{F.\,Sergiampietri}\INSTCE

%% Jyvaskyla
\author{K.\,Cankocak}\INSTJY
\author{K.\,Loo}\INSTJY
\author{J.\,Maalampi}\INSTJY
\author{G.\,Misitano}\INSTJY
\author{W.H.\,Trzaska}\INSTJY
\author{S.\,Vihonen}\INSTJY

%% Kure
\author{S.\,Kasai}\INSTKUR

%% Kyiv
\author{V.\,Aushev}\INSTKYI
\author{Y.\,Onishchuk}\INSTKYI
%
%% UCL, London
\author{M.\,Campanelli}\INSTUCL
\author{A.\,Holin}\INSTUCL
\author{L.\,Manenti}\INSTUCL
%
% Magurele, IFIN-HH
\author{M.M.\,Badoi}\INSTIFIN
\author{A.\,Balaceanu}\INSTIFIN
\author{A.M.\,Blebea-Apostu}\INSTIFIN
\author{B.M.\,Cautisanu}\INSTIFIN
\author{B.S.\,Dimitru}\INSTIFIN
\author{M.\,Gherghel-Lascu}\INSTIFIN
\author{M.C\,Gomoiu}\INSTIFIN
\author{R.M.\,Margineanu}\INSTIFIN
\author{B.\,Mitrica}\INSTIFIN
\author{T.S.\,Mosu}\INSTIFIN
\author{A.\,Munteanu}\INSTIFIN
\author{M.\,Niculescu-Oglinzanu}\INSTIFIN
\author{A.\,Saftoiu}\INSTIFIN
\author{D.L.\,Stanca}\INSTIFIN
\author{P.\,Stroescu}\INSTIFIN
\author{V.\,Toboaru}\INSTIFIN

%% Madrid CIEMAT
\author{E.\,Calvo}\INSTCIEMAT
\author{C.\,Cuesta}\INSTCIEMAT
\author{I.\,Gil-Botella}\INSTCIEMAT
\author{S.\,Jim\'enez}\INSTCIEMAT
\author{C.\,Lastoria}\INSTCIEMAT 
\author{D.\,Navas}\INSTCIEMAT 
\author{C.\,Palomares}\INSTCIEMAT
\author{D.\,Redondo}\INSTCIEMAT 
\author{L.\,Romero}\INSTCIEMAT 
\author{R.\,Santorelli}\INSTCIEMAT
\author{A.\,Verdugo}\INSTCIEMAT


%% OMEGA, Palaiseau
\author{S.\,Conforti}\INSTOMEGA
\author{C.\,De La Taille}\INSTOMEGA
\author{F.\,Dulucq}\INSTOMEGA
\author{G.\,Martin-Chassard}\INSTOMEGA

% LPNHE, Paris 
\author{J.\,Dumarchez}\INSTPARIS
\author{C.\,Giganti}\INSTPARIS
\author{B.\,Popov}\INSTPARIS
\author{L.\,Scotto Lavina}\INSTPARIS

% APC, Paris
\author{J.\,Dawson}\INSTAPC
\author{P.\,Gorodetzky}\INSTAPC
\author{D.\,Kryn}\INSTAPC
\author{A.\,Noury}\INSTAPC
\author{T.\,Patzak}\INSTAPC
\author{C.\,Santos}\INSTAPC
\author{A.\,Scarpelli}\INSTAPC
\author{A.\,Tonazzo}\INSTAPC
\author{F.\,Vannucci}\INSTAPC

%% Princeton
\author{C.~Galbiati}\INSTPRIN
\author{K.T.~McDonald}\INSTPRIN
\author{W.R.~Sands}\INSTPRIN

% CEA-Saclay
\author{S.\,Bolognesi}\INSTJ
\author{Ph. Cotte}\INSTJ
\author{A.\,Delbart}\INSTJ
\author{S. Emery}\INSTJ
\author{M. Karolak}\INSTJ
\author{E. Mazzucato}\INSTJ
\author{Y. Penichot}\INSTJ
\author{G. Vasseur}\INSTJ
\author{M.\,Zito}\INSTJ

%% KEK Tsukuba
\author{E.\,Hamada}\INSTKEK
\author{T.\,Hasegawa}\INSTKEK
\author{M.\,Ikeno}\INSTKEK
\author{K.\,Kasami}\INSTKEK
\author{T.\,Kishishita}\INSTKEK
\author{M.\,Maki}\INSTKEK
\author{K.\,Nakayoshi}\INSTKEK
\author{K.\,Sakashita}\INSTKEK
\author{K.\,Sendai}\INSTKEK
\author{M.\,Shoji}\INSTKEK
\author{M.\,Tanaka}\INSTKEK
\author{T.\,Uchida}\INSTKEK


% IPN Lyon, Villeurbanne
\author{D.\,Autiero}\INSTE
\author{E.\,Bechetoille}\INSTE
\author{L.\,Balleyguier}\INSTE
\author{D.\,Caiulo}\INSTE
\author{B.\,Carlus}\INSTE
\author{F.\,Doizon}\INSTE
\author{V.\,Galymov}\INSTE
\author{C.\,Girerd}\INSTE
\author{J.\,Marteau}\INSTE
\author{H.\,Mathez}\INSTE
\author{E.\,Pennacchio}\INSTE
\author{W.\,Tromeur}\INSTE
\author{D.\,Pugnere}\INSTE

%% NCBJ
\author{D.~Stefan}\INSTNCBJ
\author{R.~Sulej}\INSTNCBJ


%% Iwate
\author{L.\,Aizawa}\INSTIWA
\author{H.\,Konari}\INSTIWA
\author{M.\,Kurokawa}\INSTIWA
\author{Y.\,Kuromori}\INSTIWA
\author{S.\,Narita}\INSTIWA
\author{K.\,Negishi}\INSTIWA

% ETHZ
\author{Ch.~Alt}\INSTA
\author{C.~Cantini}\INSTA
\author{P.~Chiu}\INSTA
\author{P.~Crivelli}\INSTA
\author{K.~Fusshoeller}\INSTA
\author{A.~Gendotti}\INSTA
\author{S.~Horikawa}\INSTA
\author{L.\,Molina Bueno}\INSTA
\author{S.~Murphy}\INSTA
\author{L.~Periale}\INSTA
\author{B.\,Radics}\INSTA
\author{C.~Regenfus}\INSTA
\author{A.~Rubbia}\INSTA
\author{C.~Schloesser}\INSTA
\author{T.~Viant}\INSTA
\author{M.~Wei}\INSTA
\author{S.~Wu}\INSTA


==> anames/AuthorListFormat2.tex <==
\author[i]{B.\,Aimard}
\author[i]{G.\,Balik}
\author[i]{L.\,Brunetti}
\author[i]{A.\,Chappuis}
\author[i]{I.\,De Bonis}
\author[i]{C.\,Drancourt}
\author[i]{D.\,Duchesneau}
\author[i]{N.\,Geffroy}
\author[i]{Y.\,Karyotakis}
\author[i]{H.\,Pessard}
\author[i]{A.\,Remoto}
\author[i]{S.\,Vilalte}
\author[i]{L.\,Zambelli}
\address[i]{LAPP, Universit\'e de Savoie, CNRS/IN2P3, Annecy-le-Vieux, France}

\author[u]{J.\,Asaadi}
\author[u]{G.\,Brown}
\author[u]{A.\,Chatterjee}
\author[u]{A.\,Falcone}
\author[u]{N.\,Lira}
\author[u]{S.\,Shahsavarani}
\author[u]{J.\,Yu}
\address[u]{University of Texas Arlington, Arlington, USA}

\author[n]{B.\,Bourguille}
\author[n]{S.\,Bordoni}
\author[n]{S.\,Di\,Luise}
\author[n]{T.\,Lux}
\author[n]{F.\,Sanchez}
\address[n]{Institut de Fisica d'Altes Energies (IFAE), Bellaterra (Barcelona), Spain}

\author[v]{G.\,Brunetti}
\address[v]{Fermilab, Batavia, IL, USA}

\author[b]{M.\,Auger}
\author[b]{A.\,Ereditato}
\author[b]{R.\,Hanni}
\author[b]{I.\,Kreslo}
\author[b]{D.\,Lorca}
\author[b]{P.\,Lutz}
\author[b]{J.\,Sinclair}
\author[b]{M.\,Weber}
\address[b]{University of Bern, Albert Einstein Center for Fundamental Physics, Laboratory for High Energy Physics (LHEP), Bern, Switzerland}

\author[f]{M.\,Calin}
\author[f]{A.\,Chiriacescuf}
\author[f]{T.\,Esanu}
\author[f]{A.\,Jipa}
\author[f]{I.\,Lazanu}
\author[f]{L.\,Nita}
\author[f]{M.\,Parvuf}
\author[f]{O.\,Ristea}
\author[f]{C.\,Ristea}
\address[f]{University of Bucharest, Faculty of Physics, Bucharest, Romania}

\author[h]{N.\,Bourgeois}
\author[h]{J.\,Bremer}
\author[h]{M.\,Chalifour}
\author[h]{N.\,Charitonidis}
\author[h]{F.\,Duval}
\author[h]{G.\,Lehmann-Miotto}
\author[h]{G.\,Maire}
\author[h]{D.\,Mladenov}
\author[h]{M.\,Nessi}
\author[h]{F.\,Noto}
\author[h]{F.\,Pietropaolo}
\author[h]{F.\,Resnati}
\author[h]{F.\,Sergiampietri}
\address[h]{CERN, Geneva, Switzerland}

\author[e]{K.\,Cankocak}
\author[e]{K.\,Loo}
\author[e]{J.\,Maalampi}
\author[e]{G.\,Misitano}
\author[e]{W.H.\,Trzaska}
\author[e]{S.\,Vihonen}
\address[e]{University of Jyv\"askyl\"a,  Department of Physics, Jyv\"askyl\"a, Finland}

\author[q]{S.\,Kasai}
\address[q]{National Institute of Technology Kure College, Kure, Hiroshima, Japan}

\author[w]{V.\,Aushev}
\author[w]{Y.\,Onishchuk}
\address[w]{Kyiv National University, Kyiv, Ukraine}

\author[l]{M.\,Campanelli}
\author[l]{A.\,Holin}
\author[l]{L.\,Manenti}
\address[l]{University College London, Dept. of Physics and Astronomy, London, United Kingdom}

\author[r]{M.M.\,Badoi}
\author[r]{A.\,Balaceanu}
\author[r]{A.M.\,Blebea-Apostu}
\author[r]{B.M.\,Cautisanu}
\author[r]{B.S.\,Dimitru}
\author[r]{M.\,Gherghel-Lascu}
\author[r]{M.C.\,Gomoiu}
\author[r]{R.M.\,Margineanu}
\author[r]{B.\,Mitrica}
\author[r]{T.S.\,Mosu}
\author[r]{A.\,Munteanu}
\author[r]{M.\,Niculescu-Oglinzanu}
\author[r]{A.\,Saftoiu}
\author[r]{D.L.\,Stanca}
\author[r]{P.\,Stroescu}
\author[r]{V.\,Toboaru}
\address[r]{Horia Hulubei National Institute of R\&D for Physics and Nuclear Engineering - IFIN-HH, Magurele, Romania}

\author[m]{D.\,Belver}
\author[m]{E.\,Calvo}
\author[m]{C.\,Cuesta}
\author[m]{A.\,Gallego-Ros}
\author[m]{I.\,Gil-Botella}
\author[m]{S.\,Jim\'enez}
\author[m]{C.\,Lastoria}
\author[m]{D.\,Navas-Nicol\'as}
\author[m]{C.\,Palomares}
\author[m]{D.\,Redondo}
\author[m]{J.\,Soto-Oton}
\author[m]{A.\,Verdugo}
\address[m]{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}

\author[s]{S.\,Conforti}
\author[s]{C.\,De La Taille}
\author[s]{F.\,Dulucq}
\author[s]{G.\,Martin-Chassard}
\address[s]{OMEGA Ecole Polytechnique/CNRS-IN2P3, Palaiseau, France}

\author[j]{J.\,Dumarchez}
\author[j]{C.\,Giganti}
\author[j]{B.\,Popov}
\author[j]{L.\,Scotto Lavina}
\address[j]{UPMC, Universit\'e Paris Diderot, CNRS/IN2P3, Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Paris, France}

\author[k]{J.\,Dawson}
\author[k]{P.\,Gorodetzky}
\author[k]{D.\,Kryn}
\author[k]{A.\,Noury}
\author[k]{T.\,Patzak}
\author[k]{C.\,Santos}
\author[k]{A.\,Scarpelli}
\author[k]{A.\,Tonazzo}
\author[k]{F.\,Vannucci}
\address[k]{AstroParticule et Cosmologie (APC), Universit\'e Paris Diderot, CNRS/IN2P3, CEA/Irfu, Observatoire de Paris, Sorbonne Paris Cit\'e, Paris, France}

\author[d]{S.\,Bolognesi}
\author[d]{Ph.\,Cotte}
\author[d]{A.\,Delbart}
\author[d]{S.\,Emery}
\author[d]{M.\,Karolak}
\author[d]{E.\,Mazzucato}
\author[d]{Y.\,Penichot}
\author[d]{G.\,Vasseur}
\author[d]{M.\,Zito}
\address[d]{IRFU, CEA Saclay, Gif-sur-Yvette, France}

\author[o]{E.\,Hamada}
\author[o]{T.\,Hasegawa}
\author[o]{M.\,Ikeno}
\author[o]{K.\,Kasami}
\author[o]{T.\,Kishishita}
\author[o]{M.\,Maki}
\author[o]{K.\,Nakayoshi}
\author[o]{K.\,Sakashita}
\author[o]{K.\,Sendai}
\author[o]{M.\,Shoji}
\author[o]{M.\,Tanaka}
\author[o]{T.\,Uchida}
\address[o]{High Energy Accelerator Research Organization (KEK), Tsukuba,  Ibaraki, Japan}

\author[c]{D.\,Autiero}
\author[c]{E.\,Bechetoille}
\author[c]{L.\,Balleyguier}
\author[c]{D.\,Caiulo}
\author[c]{B.\,Carlus}
\author[c]{F.\,Doizon}
\author[c]{V.\,Galymov}
\author[c]{C.\,Girerd}
\author[c]{J.\,Marteau}
\author[c]{H.\,Mathez}
\author[c]{E.\,Pennacchio}
\author[c]{W.\,Tromeur}
\author[c]{D.\,Pugnere}
\address[c]{Universit\'e de Lyon, Universit\'e Claude Bernard Lyon 1, IPN Lyon (IN2P3), Villeurbanne, France}

\author[g]{D.\,Stefan}
\author[g]{R.\,Sulej}
\address[g]{National Centre for Nuclear Research (NCBJ), Warsaw, Poland}

\author[p]{L.\,Aizawa}
\author[p]{H.\,Konari}
\author[p]{M.\,Kurokawa}
\author[p]{Y.\,Kuromori}
\author[p]{S.\,Narita}
\author[p]{K.\,Negishi}
\address[p]{Iwate University, Department of Electrical Engineering and Computer Science, Morioka, Iwate, Japan}

\author[a]{Ch.\,Alt}
\author[a]{C.\,Cantini}
\author[a]{P.\,Chiu}
\author[a]{P.\,Crivelli}
\author[a]{K.\,Fusshoeller}
\author[a]{A.\,Gendotti}
\author[a]{S.\,Horikawa}
\author[a]{L.\,Molina Bueno}
\author[a]{W.\,Mu}
\author[a]{S.\,Murphy}
\author[a]{L.\,Periale}
\author[a]{B.\,Radics}
\author[a]{C.\,Regenfus}
\author[a]{A.\,Rubbia}
\author[a]{C.\,Schloesser}
\author[a]{T.\,Viant}
\author[a]{S.\,Wu}
\address[a]{ETH Zurich, Institute for Particle Physics, Zurich, Switzerland}

